Identifying and Replicating Code Patterns Driving Performance Regressions in Software Systems

Context: Performance regressions negatively impact execution time and memory usage of software systems. Nevertheless, there is a lack of systematic methods to evaluate the effectiveness of performance test suites. Performance mutation testing, which introduces intentional defects (mutants) to measure and enhance fault-detection capabilities, is promising but underexplored. A key challenge is understanding if generated mutants accurately reflect real-world performance issues. Goal: This study evaluates and extends mutation operators for performance testing. Its objectives include (i) collecting existing performance mutation operators, (ii) introducing new operators from real-world code changes that impact performance, and (iii) evaluating these operators on real-world systems to see if they effectively degrade performance. Method: To this aim, we will (i) review the literature to identify performance mutation operators, (ii) conduct a mining study to extract patterns of code changes linked to performance regressions, (iii) propose new mutation operators based on these patterns, and (iv) apply and evaluate the operators to assess their effectiveness in exposing performance degradations. Expected Outcomes: We aim to provide an enriched set of mutation operators for performance testing, helping developers and researchers identify harmful coding practices and design better strategies to detect and prevent performance regressions.

==> Sections/Backup_RQs_Objectives.tex <==
\section{Research Questions and Objectives}
\label{section:Research_Design}

The \textit{goal} of the empirical study is to evaluate the effectiveness of performance mutation operators across diverse platforms and environments, with the \textit{purpose} of identifying (1) which operators are most effective at exposing performance slowdowns in specific environmental (e.g., workload intensity) and platform contexts (e.g., JVMs implementations and operational systems), and (2) the conditions under which the operators provide the most actionable insights into potential performance issues. The \textit{perspective} is of researchers interested in understanding performance mutation under specific conditions, developers interested in practical insights to enhance their debugging and optimization workflows, and tool creators aiming to design tools that assist in detecting and resolving performance problems more efficiently.

More specifically, our empirical investigation will first aim at addressing the following research questions (\textbf{RQ}s):

\resquestion{1}{Which performance mutation operators are most effective at identifying performance slowdowns under different environmental contexts?}

\resquestion{2}{Which performance mutation operators are most effective at identifying performance slowdowns under different platform-specific configurations?}

Through \textbf{RQ$_{1}$} and \textbf{RQ$_{2}$}, we aim to address the first objective of the study. In \textbf{RQ$_{1}$}, we investigate the effectiveness of performance mutation operators for different application domains and workload intensity. In \textbf{RQ$_{2}$}, we investigate the effectiveness of performance mutation operators under different JVM implementations. The understanding of which mutation operators have the highest diagnostic value could inform (1) the factors that are associated with the effectiveness of mutants in specific contexts and (2) the design of novel or improved instruments to better support developers in identifying and resolving performance issues. For instance, should we discover that certain mutants are rarely effective under specific platform configurations, this would imply that further research is needed to refine mutation designs to account for platform-specific constraints. %These findings will not only advance theoretical knowledge of performance mutation but also offer practical guidance for developers and tool creators, enabling them to address performance issues with greater precision and efficiency.

Upon completion of this investigation, we will further elaborate on the on the optimization of mutants to enhance their efficacy in identifying system slowdowns across diverse platforms and environments, addressing the following research question:

\resquestion{3}{How can mutants be tailored or optimized to enhance their ability to identify slowdowns across a range of platforms and environments?}

Some performance issues may consistently manifest across different environments or platforms. For example, a mutation may have negligible impact on single- or multi-core platforms under low workloads. Identifying these can provide a baseline set of "environment-agnostic" mutants for robust testing. On the other hand, Not all mutants will be equally important in every environment. For example, a mutation that affects memory use might be irrelevant for server applications but critical for embedded systems. Studying the intersection of these dimensions provides a holistic view, helping to identify mutants that reveal real-world performance vulnerabilities. This combined perspective can guide the creation of benchmarks or testing tools that are environment- and platform-aware or even dependent.
%taxonomy of platform-dependent factors 
%Introduce environment-aware mutation testing





Jangali et al. \cite{jangali2022automated} conducted the implementation of a framework called ju2jmh, which automatically converts unit tests (JUnit) into microbenchmarks to evaluate code performance. The goal is to analyze the quality of these automatically generated microbenchmarks, using mutation tests as the evaluation method. The comparison is made on three levels: (i) benchmarks generated by ju2jmh, (ii) benchmarks created manually with JMH (Java Microbenchmark Harness), and (iii) benchmarks generated automatically by another tool called AutoJMH. In addition, the ju2jmh results are compared directly with performance measurements made by the JUnit tests themselves, highlighting the differences between these approaches in evaluating system performance. The results indicated that JMH benchmarks generated by ju2jmh consistently perform better in terms of execution time and throughput when compared to using JUnit tests as a performance proxy, as well as JMH benchmarks automatically generated by the AutoJMH tool. In addition, the benchmarks generated by ju2jmh demonstrate a stability and performance fault detection capability comparable to JMH benchmarks written manually by developers.\looseness=-1

Wang et al. \cite{wang2024exploratory} conducted a large-scale study to investigate the performance of six LLMs in generating traditional mutants in in terms of cost, usability (i.e., compilability rate, useless mutation rate, and equivalent mutation rate, AST node diversity), and behavior similarity with real bugs. The authors utilized 851 bugs from two Java benchmarks (Defects4J 2.0 and ConDefects). The results indicate that the GPT-4 models excel at generating mutations that closely mimic real bugs.The authors analyzed the types of non-compilable mutation errors. In addition, the authors adopted some evaluation metrics such as Cost Metric, Usability Metrics, and Behavior.

Tip et al. \cite{tip2024llmorpheus} developed a tool called LLMorpheus. The tool presents an LLM-based technique for traditional mutation testing for JavaScript,  and evaluated on 13 subject packages, considering several variations on the prompting strategy, and using several LLMs. The results pointed out that LLMorpheus is capable of producing mutants that resemble real bugs that cannot be produced using standard mutation operators. In addition, the study indicates that most of the surviving mutants (63\%) are behavioral changes, and that the number of (almost) equivalent mutants is less than 20\%.

In summary, our study first investigates whether developers rely on benchmarks (performance tests) to identify slowdowns and check whether fixes effectively solve problems. In addition, we sought to evaluate the generalizability of performance mutation operators in different contexts, something that has been little explored. Unlike related work that prioritizes functional mutants or benchmark automation, our work aims to prioritize, identify and model real performance problems.



==> Sections/Results.tex <==
\section{Results}
\label{section:results}
